The Bricklayer Ecosystem - Art, Math, and Code

This paper describes the Bricklayer Ecosystem - a freely-available online educational ecosystem created for people of all ages and coding backgrounds. Bricklayer is designed in accordance with a "low-threshold infinite ceiling" philosophy and has been successfully used to teach coding to primary school students, middle school students, university freshmen, and in-service secondary math teachers. Bricklayer programs are written in the functional programming language SML and, when executed, create 2D and 3D artifacts. These artifacts can be viewed using a variety of third-party tools such as LEGO Digital Designer (LDD), LDraw, Minecraft clients, Brickr, as well as STereoLithography viewers.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{J. Jeuring and J. McCarthy (Eds.): Trends in\\
Functional Programming in Education (TFPIE)\\
EPTCS 230, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.230.4}{10.4204/EPTCS.230.4}}
\pdfoutput=1

